Learning from {\L}ukasiewicz and Meredith: Investigations into Proof Structures (Extended Version)

The material presented in this paper contributes to establishing a basis deemed essential for substantial progress in Automated Deduction. It identifies and studies global features in selected problems and their proofs which offer the potential of guiding proof search in a more direct way. The studied problems are of the wide-spread form of "axiom(s) and rule(s) imply goal(s)". The features include the well-known concept of lemmas. For their elaboration both human and automated proofs of selected theorems are taken into a close comparative consideration. The study at the same time accounts for a coherent and comprehensive formal reconstruction of historical work by {\L}ukasiewicz, Meredith and others. First experiments resulting from the study indicate novel ways of lemma generation to supplement automated first-order provers of various families, strengthening in particular their ability to find short proofs.

==> cmproof_expanded_02_xy.tex <==
\matrix[column sep=0.5em,row sep=0.4em] (m1) at (14.700000000000001,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{1}\\[\cmfiginl]
   \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_1y_1\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_1\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_1\&\rule[-1ex]{0pt}{3ex}\f{P}g\nhphantom{$\f{P}g$}\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m2) at (12.25,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{2}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_1 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_2y_2\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_2 \& \rule[-1ex]{0pt}{3ex}\f{P}x_2\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_2\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m3) at (9.8,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{3}\\[\cmfiginl]
   \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_3y_3\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_3\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_3\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m4) at (7.3500000000000005,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{4}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_3 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_4y_4\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_4\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_4\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m5) at (4.9,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{5}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_4 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_5y_5\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_5 \& \rule[-1ex]{0pt}{3ex}\f{P}x_5\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_5\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m6) at (2.45,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{6}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_6 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_6y_6\\
   \& \rule[-1ex]{0pt}{3ex}\f{P}x_6\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_6\\
};

\matrix[column sep=0.5em,row sep=0.4em] (m7) at (0.0,1) [ampersand replacement=\&,matrix of math nodes]
{ \& \cmfiginst{7}\\[\cmfiginl]
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_7 \& \rule[-1ex]{0pt}{3ex}\f{P}\f{i}x_7y_7\\
  \rule[-1ex]{0pt}{3ex}\lnot \f{P}a_8 \& \rule[-1ex]{0pt}{3ex}\f{P}x_7\\
   \& \rule[-1ex]{0pt}{3ex}\lnot \f{P}y_7\\
};

\draw[] (m1-4-2) edge node [midway,above] {\cmfigconn{1}} (m1-4-3);
\draw[] (m1-2-2.west) edge[in=85,out=220,looseness=1.1] node [pos=0.4,left] {\cmfigconn{2}} (m2-4-2.east);
\draw[] (m1-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m3-4-2.east);
\draw[] (m2-2-1) edge node [midway,above] {\cmfigconn{4}} (m2-2-2);
\draw[] (m2-3-1) edge node [midway,above] {\cmfigconn{5}} (m2-3-2);
\draw[] (m3-2-2.west) edge[in=85,out=220,looseness=1.1] node [pos=0.4,left] {\cmfigconn{2}} (m4-4-2.east);
\draw[] (m3-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m6-4-2.east);
\draw[] (m4-2-1) edge node [midway,above] {\cmfigconn{4}} (m4-2-2);
\draw[] (m4-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m5-4-2.east);
\draw[] (m5-2-1) edge node [midway,above] {\cmfigconn{4}} (m5-2-2);
\draw[] (m5-3-1) edge node [midway,above] {\cmfigconn{5}} (m5-3-2);
\draw[] (m6-2-1) edge node [midway,above] {\cmfigconn{4}} (m6-2-2);
\draw[] (m6-3-2.west) edge[in=-40,out=250,looseness=1.1] node [midway,above] {\cmfigconn{3}} (m7-4-2.east);
\draw[] (m7-2-1) edge node [midway,above] {\cmfigconn{4}} (m7-2-2);
\draw[] (m7-3-1) edge node [midway,above] {\cmfigconn{5}} (m7-3-2);

